Distribution of Quantum Circuits Over General Quantum Networks

Near-term quantum computers can hold only a small number of qubits. One way to facilitate large-scale quantum computations is through a distributed network of quantum computers. In this work, we consider the problem of distributing quantum programs represented as quantum circuits across a quantum network of heterogeneous quantum computers, in a way that minimizes the overall communication cost required to execute the distributed circuit. We consider two ways of communicating: cat-entanglement that creates linked copies of qubits across pairs of computers, and teleportation. The heterogeneous computers impose constraints on cat-entanglement and teleportation operations that can be chosen by an algorithm. We first focus on a special case that only allows cat-entanglements and not teleportations for communication. We provide a two-step heuristic for solving this specialized setting: (i) finding an assignment of qubits to computers using Tabu search, and (ii) using an iterative greedy algorithm designed for a constrained version of the set cover problem to determine cat-entanglement operations required to execute gates locally. For the general case, which allows both forms of communication, we propose two algorithms that subdivide the quantum circuit into several portions and apply the heuristic for the specialized setting on each portion. Teleportations are then used to stitch together the solutions for each portion. Finally, we simulate our algorithms on a wide range of randomly generated quantum networks and circuits, and study the properties of their results with respect to several varying parameters.

==> GeneralizedProblem.tex <==
\section{\gdqc Problem}\label{sec:generalized_Problem}

 In the \gdqc problem, we seek to distribute a quantum circuit across quantum computers of varying qubit and ebit-storage capacities in a manner that minimizes the overall communication cost. 

Note that cuts portion the input circuit into several sub-circuits with varying initial qubit-assignments. We pass each such sub-circuit to the Iterative Max-$k$-Cover algorithm presented in section \ref{sec:mdqcproblem} to obtain a set of migrations that cover all CZ gates in the sub-circuit. Finally, we merge migrations that remain the same across adjacent cuts.  

Thus, an initial partition, along with migrations and teleportations that cover all CZ gates form a solution of the \dqc problem. The cost of such a solution depends on the number of migrations and teleportations.

\begin{definition}[Communication Cost]
Given a collection of migrations $\mathcal{M}=\{M_1,M_2,\dots , M_r\}$ and a collection of teleportations $\mathrm{T}=\{\tau _1, \tau_2,\dots , \tau_s\}$ corresponding to a quantum circuit, the total communication cost of the circuit is $\mathcal{C}= \sum \limits _{i=1}^ r cost(M_i)+ \sum _{j=1}^s cost(\tau_j)$.  
\end{definition}



\para{\gdqc Problem Formulation.} 
Let $C=\{Q, \{g_1,g_2, \dots , g_m\}\}$ be a quantum circuit, $P=\{P_1, P_2, \dots ,P_p\}$ be a network topology of quantum computers with qubit storage capacities $[a_1, a_2, \dots, a_p]$ and execution memory constraints $[b_1, b_2, \dots, b_p]$. The objective of the \gdqc problem is to determine an initial assignment of the qubits to computers, along with a sequence of feasible migrations and teleportations that cover all the non-local CZ gates, while minimizing the total communication cost. 

\subsection{Overall Algorithm}

Our overall algorithm runs Sequence and Split algorithms for each input, and chooses the set of cuts with lower cost. Once we obtain the cuts, we run Tabu search and Iterative Max-$k$-Cover algorithms on each of the portions to obtain migrations that cover all CZ gates and teleportations that change the home-computers of qubits. 

\floatname{algorithm}{Algorithm}
\begin{algorithm}[h]
\caption{Overall Algorithm}
  \label{alg:Overall}  
  \begin{flushleft}
  \textbf{Input:}  A circuit $C$ over qubits $Q$, a network graph $G=(v_1, v_2, \dots, v_p)$ and a vector of qubit storage capacities $\mathcal{A}=[a_1,\dots, a_p]$ and ebit memory constraints $\mathcal{B}=[b_1,\dots b_p]$. Let $\mathcal{T}=\{1,\dots, m\}$ be the indices of the CZ gates in $C$.  \\
  \textbf{Output:} An initial assignment of qubits to computers called $partition$, a set of migrations $\mathcal{M}$ and a set of teleportations $\mathrm{T}$.
  \end{flushleft}
  \begin{algorithmic}
        \STATE Split cuts= Split Algorithm($C$, $Q$, $G$)
        \STATE Sequence cuts= Sequence Algorithm($C$, $Q$, $G$)
        \STATE Best cuts = $argmin_{cost}$(Split cuts, Sequence cuts)
        \STATE $\mathcal{M}, \mathcal{T} = \emptyset$.
        \STATE initial partition= \textsc{Tabu Search} ($C[0:$Best cuts[0] $],G, \mathcal{A}, \mathcal{B}$).
        \STATE $\mathcal{M}_0$ = \textsc{IterativeMaxkCover}($C$[0:Best cuts[0]], initial partition, $\mathcal{B}$)
        \STATE previous partition = initial partition
        \FOR{ $i$ in Best cuts[1:]}
        \STATE partition= \textsc{Tabu Search} ($C[i-1: i],G, \mathcal{A}, \mathcal{B}$).
        \STATE $\mathcal{M}_{i}$= \textsc{IterativeMaxkCover}($C[i-1: i]$, partition, $\mathcal{B}$)
        \STATE $\mathcal{T}_i$= teleportations(previous partition, partition)
        \STATE $\mathcal{M} \leftarrow \mathcal{M} \cup \mathcal{M}_i$, $\mathcal{T} \leftarrow \mathcal{T} \cup \mathcal{T}_i$.
        \ENDFOR
        \RETURN initial partition, $\mathcal{M}, \mathcal{T}$.
  \end{algorithmic}
  \label{alg:hc}
\end{algorithm}
